Multi-Frame Super-Resolution Reconstruction with Applications to Medical Imaging

The optical resolution of a digital camera is one of its most crucial parameters with broad relevance for consumer electronics, surveillance systems, remote sensing, or medical imaging. However, resolution is physically limited by the optics and sensor characteristics. In addition, practical and economic reasons often stipulate the use of out-dated or low-cost hardware. Super-resolution is a class of retrospective techniques that aims at high-resolution imagery by means of software. Multi-frame algorithms approach this task by fusing multiple low-resolution frames to reconstruct high-resolution images. This work covers novel super-resolution methods along with new applications in medical imaging.

==> d-cov.tex <==
%auto-ignore

% -----------------------------------------------------
% D-TITEL.TEX zur Verwendung mit TEXPART
% (an eigene Gegebenheiten anzupassen)
% -----------------------------------------------------
%
\pdfbookmark[1]{Cover}{cov}
\begin{titlepage}
\centering
\huge
\vspace*{\fill}
%-----------
Multi-Frame Super-Resolution Reconstruction with Applications to Medical Imaging\\
\vspace{1cm}
Thesis Title in German 
\vspace{2cm}\\
%-----------
\Large
Der Technischen Fakult\"at\\
der Friedrich-Alexander-Universit\"at\\
Erlangen-N\"urnberg \vspace{1.5cm}\\
%-----------
zur\vspace{1cm}\\
\huge
Erlangung des Doktorgrades Dr.-Ing.  \vspace{1cm}\\
\Large
%-----------
vorgelegt von \vspace{2cm}\\

Thomas K\"ohler\\
aus\\
Bamberg
%-----------
\vspace*{\fill}
\end{titlepage}

\newpage
{
\large
\thispagestyle{empty}
\vspace*{\fill}
\begin{center}
Als Dissertation genehmigt\\
von der Technischen Fakult"at\\
der Friedrich-Alexander-Universit\"at Erlangen-N\"urnberg \\
\begin{tabular}{p{8cm}p{8cm}}
\rule{4.8cm}{0pt} & \rule{5.8cm}{0pt} \\
Tag der m\"undlichen Pr\"ufung:   			& \\
Vorsitzende des Promotionsorgans: & Prof. Dr. Peter Greil\\
Gutachter: 												& Prof. Dr.-Ing. Joachim Hornegger\\
																	& Prof. Dr.-Ing. Andreas Maier\\
\end{tabular}
\end{center}
}
\vspace*{1cm}


==> d-idx.tex <==
%auto-ignore

\phantomsection
\addcontentsline{toc}{chapter}{Index}
\printindex
\cleardoublepage


==> d-loa.tex <==
%auto-ignore

\phantomsection
\addcontentsline{toc}{chapter}{List of Algorithms}
\listofalgorithms
\cleardoublepage

